Evaluating Micro Parsons Problems as Exam Questions

Parsons problems are a type of programming activity that present learners with blocks of existing code and requiring them to arrange those blocks to form a program rather than write the code from scratch. Micro Parsons problems extend this concept by having students assemble segments of code to form a single line of code rather than an entire program. Recent investigations into micro Parsons problems have primarily focused on supporting learners leaving open the question of micro Parsons efficacy as an exam item and how students perceive it when preparing for exams. To fill this gap, we included a variety of micro Parsons problems on four exams in an introductory programming course taught in Python. We use Item Response Theory to investigate the difficulty of the micro Parsons problems as well as the ability of the questions to differentiate between high and low ability students. We then compare these results to results for related questions where students are asked to write a single line of code from scratch. Finally, we conduct a thematic analysis of the survey responses to investigate how students' perceptions of micro Parsons both when practicing for exams and as they appear on exams.

==> imgs/prefs.tex <==
\begin{tikzpicture}
    \pgfplotstableread{
Agree      MicroPref    Neutral       StatementPref
Exam       42.0         22.0          36.0
Practice   24.0         41.0          35.0
    }\frequency
    \begin{axis}[
        scale only axis,
        name=ax1,
        legend cell align=center,
        legend columns=-1,
        legend style={at={(1,-0.25)},anchor=north,draw=none},
        xbar stacked,
        xmin=-100,
        xmax=0,
        try min ticks=3,
        xticklabel style = {font=\scriptsize},
        xticklabel=\pgfmathparse{abs(\tick)}\pgfmathprintnumber{\pgfmathresult}\,$\%$,
        ytick=data,
        yticklabel style={align=center},
        yticklabels={
          Exams,
          Practice
        },
        enlarge y limits={abs=0.45cm},
        width=75px,
        height=60px
    ]
        \addlegendimage{fill=yellow}
        \addlegendimage{fill=gray!70!blue!10}
        \addlegendimage{fill=blue}
        \addplot [fill=gray!70!blue!10] table [x expr=-(\thisrow{Neutral}/2), meta=Agree ,y expr=\coordindex] {\frequency};
        \addplot [fill=yellow!90] table [x expr=-\thisrow{MicroPref}, meta=Agree ,y expr=\coordindex] {\frequency};
        \addlegendentry{MicroParsons\ \ }
        \addlegendentry{No Preference\ \ }
        \addlegendentry{Single-Line Code Writing} 
    \end{axis}

    \begin{axis}[
        scale only axis,
        at=(ax1.south east),
        xbar stacked,
        xmin=0,
        xmax=100,
        xticklabel style = {font=\scriptsize},
        try min ticks=3,
        xticklabel=\pgfmathparse{abs(\tick)}\pgfmathprintnumber{\pgfmathresult}\,$\%$,
        ytick=data,
        yticklabels={},
        enlarge y limits={abs=0.45cm},
        width=75px,
        height=60px
    ]

        \addplot [fill=gray!70!blue!10] table [x expr=(\thisrow{Neutral}/2), meta=Agree ,y expr=\coordindex] {\frequency};
        \addplot [fill=blue] table [x=StatementPref, meta=Agree ,y expr=\coordindex] {\frequency};

    \end{axis}
    \vspace{-3mm}
\end{tikzpicture}

